TP-RAG: Benchmarking Retrieval-Augmented Large Language Model Agents for Spatiotemporal-Aware Travel Planning

Large language models (LLMs) have shown promise in automating travel planning, yet they often fall short in addressing nuanced spatiotemporal rationality. While existing benchmarks focus on basic plan validity, they neglect critical aspects such as route efficiency, POI appeal, and real-time adaptability. This paper introduces TP-RAG, the first benchmark tailored for retrieval-augmented, spatiotemporal-aware travel planning. Our dataset includes 2,348 real-world travel queries, 85,575 fine-grain annotated POIs, and 18,784 high-quality travel trajectory references sourced from online tourist documents, enabling dynamic and context-aware planning. Through extensive experiments, we reveal that integrating reference trajectories significantly improves spatial efficiency and POI rationality of the travel plan, while challenges persist in universality and robustness due to conflicting references and noisy data. To address these issues, we propose EvoRAG, an evolutionary framework that potently synergizes diverse retrieved trajectories with LLMs' intrinsic reasoning. EvoRAG achieves state-of-the-art performance, improving spatiotemporal compliance and reducing commonsense violation compared to ground-up and retrieval-augmented baselines. Our work underscores the potential of hybridizing Web knowledge with LLM-driven optimization, paving the way for more reliable and adaptive travel planning agents.

==> sections/abstract_old_1.tex <==
\begin{abstract}
Large language models (LLMs) agents have powered the automation of travel planning but struggle with nuanced spatiotemporal coherence and the quality of Points of Interest (POIs).
Due to rich travel-domain documents on the Web, this paper explores whether LLM agents can leverage online knowledge for spatiotemporal-aware travel planning.
We introduce \textbf{\textit{TravelPlanRAG}}, the first benchmark tailored for this purpose, featuring a real-world dataset that encompasses fine-grained spatiotemporal POI attributes and plentiful reference plans sourced from the Web.
Extensive experiments demonstrate the potential of integrating Web knowledge, while also revealing concerns regarding universality and robustness.
To address these challenges, we develop \textbf{\textit{EvoTravel}}, an evolutionary optimization framework that harmonizes multifarious retrieved knowledge with LLMs' internal reasoning and exhibits greater resilience to quality deficiency, achieving superior performance in spatiotemporal rationality.
\end{abstract}


==> sections/benchmark_old_1.tex <==
\section{TravelPlanRAG}

\begin{figure*}[ht]
\centering
\includegraphics[width=\textwidth]{figs/main.png}
\vspace{-18pt}
\caption{Dataset construction pipeline.}
\vspace{-15pt}
\label{figure:main}
\end{figure*}

\subsection{Problem Definition}

In this section, we present a formal introduction to our proposed travel planning problem. 
To validate the spatiotemporal planning capabilities of LLM agents, we simplify the travel planning problem into the generation of a single-city, multi-day travel itinerary comprising attraction POIs.
Also we adopt a sole-planning mode that obviates the need for tool calls, thereby exclusively assessing the planning skills of the agents~\cite{xie2024travelplanner}.
We delineate two paradigms of the travel planning problem below:
% In contrast to prior works such as TravelPlanner~\cite{xie2024travelplanner}, our focus is directed towards validating the spatiotemporal planning capabilities of LLM agents. 
% To this end, we simplify the travel planning problem into the generation of a single-city, multi-day travel itinerary comprising attraction POIs.
% Also, we adopt a sole-planning mode that obviates the need for tool calls, thereby exclusively assessing the planning skills of the agents~\cite{xie2024travelplanner}.
% We delineate two paradigms of the travel planning problem below:

\begin{prob}
\textbf{Ground-up Spatiotemporal Travel Planning}. 
Given a travel request $r$ articulated in natural language along with pre-determined POI candidates $\mathcal{P}=\{p_i\}_{i=1}^{N}$, the LLM agent $\mathcal{L}$ selects a subset of POIs and organizes them into a plan $I=[(p_1,t_1),(p_2,t_2),...,(p_M,t_M)]$ via $I\sim\mathcal{L}(r,\mathcal{P})$, where $t$ denotes the scheduled visiting period. 
The generated plan $I$ is expected to align with the request $r$ while maximizing spatiotemporal coherence and POI semantic quality.
\end{prob}

\begin{prob}
\textbf{Retrieval-augmented Spatiotemporal Travel Planning}. 
Given a travel request $r$, POI candidates $\mathcal{P}=\{p_i\}_{i=1}^{N}$, and external knowledge $\mathcal{K}=\{k_i\}_{i=1}^{M},\ k_i=[p_1,p_2,...,p_{|k_i|}]$ consisting of online itineraries, the LLM agent $\mathcal{L}$ refer to and refine these itineraries to derive a plan $I=[(p_1,t_1),(p_2,t_2),...,(p_M,t_M)]$ via $I\sim\mathcal{L}(r,\mathcal{P}, \mathcal{C})$. 
The generated plan $I$ is expected to align with the request $r$ while maximizing spatiotemporal coherence and POI semantic quality.
\end{prob}

\subsection{Dataset Construction Pipeline}
\label{section:data}

% While the TravelPlanner series~\cite{xie2024travelplanner} has made datasets accessible for travel planning, the complexity of the requests poses challenges in gathering exactly relevant online itineraries tailored to user demands.
% To effectively explore the integration of online knowledge, it becomes imperative to construct a new dataset that emphasizes a strong correlation between requests and the information retrieved from the Web.
% Consequently, we focus on scenarios that utilize short travel requests, encompassing only the city name, travel duration, and simple soft constraints, which can be readily employed to fetch pertinent online itineraries through advanced search engines.
% The dataset construction pipeline is demonstrated in \figref{figure:main} and we will discuss each procedures below.

While the TravelPlanner series~\cite{xie2024travelplanner} has advanced the accessibility of datasets for travel planning, its reliance on highly complex user requests diverges from real-world scenarios where travelers often initiate their planning with concise, under-specified queries. 
For instance, users frequently express needs through brief inputs like "3 days in Beijing with a relaxed schedule" in search engines, expecting systems to infer and fulfill implicit requirements.
To bridge this gap between idealized planning tasks and practical applications, our benchmark prioritizes short, realistic requests which mirror common user behavior while enabling precise alignment with Web itineraries retrievable via search engines.
The dataset construction pipeline is detailed in \figref{figure:main}, with detailed procedures discussed below.

\noindent\textbf{Request Data Construction.} 
Utilizing the seed query examples sampled from Baidu searchB\footnote{\url{https://www.baidu.com}}, one of China’s largest search engines. sessions in January 2025, we engage LLMs to elaborate a comprehensive request formulation rule. 
Each request comprises several fundamental elements, including the city name, travel duration, and specific soft constraints that reflect user preferences. 
The latter two elements are optional, allowing for adjustments that control the complexity and categorization of travel requests.
In detail, The travel duration is delineated to include 3, 4, or 5 days, thereby necessitating proficient long-horizon reasoning and planning capabilities.
Soft constraints can be classified into various categories: season, holiday, POI category, traveler category, and trip compactness, as detailed in 	\tabref{table:constraint}. These constraints necessitate a robust understanding of user intent and preferences.

Based on the above standard, we further distinguish our requests into \textit{(1) generic requests} and \textit{(2) personal requests}, depending on the inclusion of soft constraints. 
Beyond generic spatiotemporal coherence, personal travel plans emphasize alignment with the original query specifications. 
Drawing on rankings provided by Sohu Travel\footnote{\url{https://travel.sohu.com/}}, we employ LLMs to create comprehensive request data for the top 30 popular cities in mainland China (\appref{appendix:city}), and summarize the statistical characteristics of the request data in \tabref{table:request}.

\noindent\textbf{POI Data Collection.}
In this phase, we traverse all predetermined requests to gather the associated attraction POIs that serve as candidates for travel planning. 
Specifically, for each request, we first exploit Large Language Models (LLMs) to reformulate the original request into several sub-requests that target attraction searches, ensuring that the queries are specifically tailored to yield relevant results. 
Subsequently, we curate these sub-requests and leverage the proprietary Baidu Search API\footnote{The Search API will be detailed in \appref{appendix:api}.} to recall web pages related to attraction recommendations, specifically targeting ten pages for each request. 
Each retrieved page is then processed through LLMs for attraction extraction, culminating in the collection of pertinent POI data for the assigned request.

\noindent\textbf{Retrieval Data Collection.}
For each request, we similarly apply query rewriting techniques and harness the Baidu Search API to directly retrieve off-the-shelf online articles that may act as references for travel planning. 
In specific, we gather twenty web documents for each query, ensuring that these documents are sourced from sessions conducted in February 2025 to maintain timeliness. To address concerns related to user privacy, full articles are not disclosed in our dataset. 
Instead, we implement a desensitization method aimed at potential open-sourcing, wherein content irrelevant to travel itineraries is filtered out by LLMs from the original documents. 
In instances where an article contains no expected itinerary information, the LLM is instructed to abstain from providing a response.

Moreover, to simulate the retrieval-augmented planning scenario for each request independently, it is essential that the attractions featured in the retrieved itineraries be included in the candidate POI data. 
Thus, we derive any unseen POIs present in the online content and incorporate them into the candidate POI set.

\noindent\textbf{Data Quality Enhancement.}
This procedure aims to ensure the quality of the generated dataset by purifying POI information and filtering out substandard data instances. 
In particular, we identify two primary issues within the POI data collected by LLMs: (1) the absence of spatiotemporal contexts for the POIs, which are crucial for effective planning, and (2) the presence of noisy information, including hallucinated POIs, non-attraction POIs, and duplicate entries.

To address these challenges, we implement a two-stage POI refinement approach using Baidu Map API\footnote{\url{https://lbsyun.baidu.com/}} in conjunction with LLMs. Initially, the Baidu Map APIs are employed to convert diverse POIs into verified locations with standardized names and enhance them with complete address, geocoordinates and shopping hours information. 
During this process, nonexistent or verbose POIs are removed from the dataset. 
However, relying solely on mapping tools does not fully eliminate semantic noise. Drawing inspiration from the assertion that judging is significantly easier than generating~\cite{wang2024omnieval}, we further make use of LLMs for data denoising by individually verifying the correctness of each POI.

In the main experiments, We retain the noise present in the itinerary data to accurately emulate the disturbances commonly found in real-world scenarios. 
We also prepared a denoised version of the retrieval data, utilized for more in-depth analysis on noise sensitivity in \secref{section:rag}.
Moreover, due to the complexity of certain travel queries, it is often difficult to gather substantial online knowledge, thereby instances with fewer than eight valid retrieved itineraries are discarded from our dataset.

\noindent\textbf{Spatiotemporal Tagging.}
Following the purification process of POI data, each POI is verified to be legitimate and tagged with essential information, including name, address, geocoordinates, and shopping hours. 
However, effective spatiotemporal travel planning requires the incorporation of fine-grained temporal information and contextual semantics. 
Therefore, we utilize LLMs augmented by Baidu Search, which can retrieve POI-level documents related to requests and summarize nuanced insights. 
These insights embrace recommended visiting periods, expected visit durations, and detailed narratives at the POI level, facilitate the utility of spatiotemporal evidence for planning.

To conclude, our dataset consists of 2,348 travel requests across 30 Chinese cities, including 115 generic requests and 2,233 personal requests that cover 5 types of soft constraints. 
This dataset is associated with 85,575 attraction POIs (averaging 36.45 POIs per request), derived from 5,018 unique attractions, and includes 18,784 retrieved itineraries (averaging 8 itineraries per request). 
Throughout the data construction process, we utilized GPT-4o~\cite{hurst2024gpt}, and the prompts employed are presented in \appref{appendix:prompt_data_generation}.
% It is noteworthy that our original dataset was developed in Chinese, and an English version of all requests, POI data, and online information is also provided to facilitate global research.

\subsection{Evaluation}

Beyond merely measuring the compliance with hard constraints in travel plans, we shed light on the nuanced aspects of generated itineraries, particularly concerning spatiotemporal rationality and the semantic prominence of POIs. 
In contrast to TripCraft~\cite{chaudhuri2025tripcraft}, we conceptualize spatiotemporal travel planning as a multi-objective optimization problem, without unique optimal solutions, thus hampering the reliability of annotating golden plans.
Following existing works, our evaluation framework integrates rule-based metrics alongside LLM-as-a-Judge methodologies, emphasizing five critical evaluation dimensions: commonsense, spatial, temporal, POI semantic and query relevance. 
This approach effectively circumvents costly annotations and mitigates potential evaluation biases, with detailed descriptions provided below.

\begin{table}[ht]
    \centering
    \vspace{-8pt}
    \caption{Metric taxonomy.}
    \vspace{-8pt}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l|l|l}
    \toprule
    \textbf{Dimension} & \textbf{Metric} & \textbf{Description}\\
    \hline
    \multirow{2}{*}{Commonsense} & FR & Legitimacy of POIs \\
    & RR & Non-redundancy of POIs. \\
    \hdashline[0.5pt/1pt]
    Spatial & DMR & Route efficiency. \\
    \hdashline[0.5pt/1pt]
    \multirow{3}{*}{Temporal} & STR & Rationality of arrival time. \\
    & DUR & Rationality of visit duration. \\
    & TBR & Comfort level of schedule. \\
    \hdashline[0.5pt/1pt]
    POI Semantic & PP & POI popularity.\\
    \hdashline[0.5pt/1pt]
    \multirow{2}{*}{Query Relevance} & PR & POI relevance. \\
    & TSR & Time schedule relevance. \\
    \bottomrule
    \end{tabular}
    }
    \vspace{-8pt}
    \label{table:metric}
\end{table}

\begin{itemize}[leftmargin=*,itemsep=2pt,topsep=0pt,parsep=0pt]
\item {\textbf{Failure Rate (FR)}: 
This metric quantifies the number of attractions absent from the candidate set, which may indicate hallucinations by the LLM agents.
}
\item {\textbf{Repetition Rate (RR)}: 
We measure the frequency of POI repetition in itineraries to assess basic commonsense awareness of the agents.
}
\item {\textbf{Distance Margin Ratio (DMR)}: 
This metric evaluates the margin ratio between the total distance required to transfer between attractions in the generated itinerary and the optimal distance determined by the Traveling Salesman Problem (TSP) solver\footnote{\url{https://github.com/fillipe-gsm/python-tsp}}.
} 
\item {\textbf{Start Time Rationality (STR)}:
It is essential to determine whether the scheduled times for visiting attractions are appropriate. 
Due to the lack of uniform standard, we prompt LLMs to consult POI-level temporal information and verify the plausibility of the scheduled arrival times through binary judgment (\ie yes or no), then calculating the total acceptable rate.
}
\item {\textbf{Duration Underflow Ratio (DUR)}:
This metric assesses how well the planned visit durations align with the expected time spans for each attraction. 
We directly used the visiting duration tags of POIs in our dataset, and then compute the average duration underflow ratio.
}
\item {\textbf{Time Buffer Ratio (TBR)}:
Given that overly tight schedules are generally inadvisable, this metric evaluates the flexibility of itineraries by estimating the proportion of buffer time available between attractions throughout the itinerary.
}
\item {\textbf{POI Popularity (PP)}:
Popular attractions are typically favored, thus, we curate LLMs to offer a golden popularity ranking based on retrieved attraction leaderboard data. 
We then calculate the top $M$ recall, where $M$ represents the number of selected POIs in the itinerary.
}
\item {\textbf{POI Relevance (PR)}:
To check the alignment of the delivered plans with the soft constraints in personal requests, we nudge LLMs to judge the matchness of each POI in a binary manner.
}
\item {\textbf{Time Schedule Relevance (TSR)}:
Similarly, LLMs are elicited to gauge whether the time intervals arranged for attractions are consistent the the personalized requirements.
}
\end{itemize}

\begin{table*}[ht]
    \centering
    % \vspace{-10pt}
    \caption{Main results (\%) of different models and strategies on our dataset. $M$ denotes the number of external itineraries we use for RAG. $R_S$, $R_T$, $R_P$, $R_R$ and $R_C$ respectively denotes the performance rank of methods from spatial, temporal, POI semantic and query relevance dimensions, and a comprehensive view averaging all aspects.}
    \vspace{-8pt}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l|cc|ccccccc|cccc|c}
    \toprule
    \textbf{Method} & \textbf{FR$\downarrow$} & \textbf{RR$\downarrow$} & \textbf{DMR$\downarrow$} & \textbf{DUR$\downarrow$} & \textbf{TBR$\uparrow$} & \textbf{STR$\uparrow$} & \textbf{PP$\uparrow$} & \textbf{PR$\uparrow$} & \textbf{TSR$\uparrow$} & $R_S\downarrow$ & $R_T\downarrow$ & $R_P\downarrow$ & $R_R\downarrow$ & $R_C\downarrow$ \\ 
    \hline
    \multicolumn{15}{c}{GPT-4o} \\ 
    \hline
    Direct & \textbf{0.32} & \textbf{0.00} & 67.92 & 3.03 & 22.01 & 77.22 & 50.82 & 80.51 & \underline{92.52} & 6.00 & 7.67 & 7.00 & \textbf{3.00} & 5.92 \\ 
    CoT & \underline{0.39} & \underline{0.01} & 69.4 & 2.78 & 22.13 & 76.96 & 50.09 & 79.92 & 91.99 & 8.00 & 8.00 & 10.00 & 6.50 & 8.12 \\ 
    Reflextion & 0.67 & 0.34 & 73.35 & 3.84 & 21.46 & 77.3 & 50.52 & 80.34 & \textbf{92.71} & 10.00 & 8.67 & 8.00 & \underline{3.50} & 7.54 \\ 
    MAC & 1.40 & 0.72 & 66.11 & 3.67 & \textbf{24.07} & 75.41 & 46.38 & \textbf{81.76} & 89.04 & 3.00 & 7.00 & 11.00 & 6.00 & 6.75 \\ 
    MAD & 0.68 & 0.07 & 74.95 & 3.68 & 20.67 & 77.14 & 50.52 & 79.53 & 92.4 & 11.00 & 9.67 & 8.00 & 6.50 & 8.79 \\ 
    \hdashline[0.5pt/1pt]
    RAG ($M$=8) & 2.05 & \underline{0.01} & 68.37 & 2.57 & \underline{23.82} & 77.19 & \underline{58.00} & \underline{80.55} & 91.58 & 7.00 & 4.67 & \underline{2.00} & 5.00 & 4.67 \\ 
    RAG ($M$=4) & 2.08 & 0.02 & 67.75 & 2.55 & 23.71 & 77.35 & 56.11 & 80.53 & 91.67 & 5.00 & 3.67 & 4.00 & 4.50 & \underline{4.29} \\ 
    RAG ($M$=1) & 2.43 & 0.04 & \underline{66.05} & 2.47 & 22.59 & 77.44 & 53.38 & 80.1 & 91.5 & \underline{2.00} & 4.00 & 6.00 & 8.50 & 5.12 \\ 
    RAG + Extr. ($M$=4) & 1.91 & 0.02 & 66.99 & \textbf{2.41} & 23.5 & \textbf{77.87} & 56.82 & 80.31 & 91.69 & 4.00 & \textbf{2.00} & 3.00 & 6.00 & \textbf{3.75} \\ 
    RAG + Extr. ($M$=1) & 2.72 & 0.06 & \textbf{65.76} & \underline{2.42} & 22.95 & \underline{77.79} & 53.85 & 80.39 & 91.64 & \textbf{1.00} & \underline{3.00} & 5.00 & 6.00 & \textbf{3.75} \\ 
    RAG + Abst. & 3.20 & 0.02 & 69.49 & 2.64 & 22.23 & 76.66 & \textbf{59.15} & 79.36 & 90.67 & 9.00 & 7.67 & \textbf{1.00} & 10.50 & 7.04 \\ 
    \hline
    \multicolumn{15}{c}{Qwen2.5-72B-Instruct} \\ 
    \hline
    Direct & \textbf{0.38} & \textbf{0.03} & 71.67 & 6.49 & 24.82 & 78.33 & 48.53 & 79.68 & 92.86 & 8.00 & \underline{5.00} & 8.00 & 9.00 & 7.50 \\ 
    CoT & \underline{0.42} & \underline{0.04} & 70.51 & 6.64 & 24.66 & 78.77 & 47.09 & 80.12 & 93.16 & 7.00 & 5.33 & 10.00 & 8.00 & 7.58 \\ 
    Reflextion & 2.39 & 1.62 & 85.38 & 8.08 & 25.37 & 77.54 & 49.15 & 79.65 & 92.14 & 10.00 & 7.67 & 7.00 & 10.00 & 8.67 \\ 
    MAC & 1.10 & 2.21 & 70.08 & \textbf{5.74} & 23.65 & 76.48 & 43.3 & \underline{81.28} & 90.00 & 6.00 & 7.33 & 11.00 & 6.50 & 7.71 \\ 
    MAD & 3.30 & 1.49 & 87.47 & 9.46 & \textbf{26.53} & 77.75 & 47.49 & 80.23 & 91.21 & 11.00 & 7.00 & 9.00 & 9.00 & 9.00 \\ 
    \hdashline[0.5pt/1pt]
    RAG ($M$=8) & 3.41 & 0.11 & 69.39 & \underline{6.35} & 23.48 & 78.4 & \underline{55.15} & \textbf{81.67} & 93.29 & 5.00 & 6.00 & \underline{2.00} & \underline{3.00} & 4.00 \\ 
    RAG ($M$=4) & 3.15 & 0.11 & 68.77 & 6.54 & 24.06 & \textbf{79.08} & 53.62 & 81.26 & \textbf{93.86} & 3.00 & \underline{5.00} & 4.00 & \textbf{2.00} & \textbf{3.50} \\ 
    RAG ($M$=1) & 2.58 & 0.09 & \textbf{68.07} & 6.89 & 25.27 & 78.48 & 51.62 & 81.07 & 93.4 & \textbf{1.00} & 5.33 & 6.00 & 4.50 & 4.21 \\ 
    RAG + Extr. ($M$=4) & 3.46 & 0.16 & 69.03 & 6.49 & 24.33 & \underline{79.03} & 54.79 & 81.21 & \underline{93.81} & 4.00 & \textbf{4.33} & 3.00 & \underline{3.00} & \underline{3.58} \\ 
    RAG + Extr. ($M$=1) & 3.16 & 0.20 & \underline{68.29} & 6.73 & \underline{25.59} & 78.33 & 52.36 & 80.92 & 93.42 & \underline{2.00} & \underline{5.00} & 5.00 & 4.50 & 4.12 \\ 
    RAG + Abst. & 3.78 & 0.17 & 72.4 & 7.32 & 25.11 & 78.04 & \textbf{56.14} & 80.5 & 93.29 & 9.00 & 7.33 & \textbf{1.00} & 6.00 & 5.83 \\
    \hline
    \multicolumn{15}{c}{LLaMA3.3-70B-Instruct} \\ 
    \hline
    Direct & \textbf{0.67} & \textbf{0.01} & 90.55 & 7.41 & 24.14 & \underline{77.07} & 46.27 & 79.75 & 89.32 & 8.00 & \underline{4.67} & 7.00 & 7.50 & 6.79 \\ 
    CoT & \underline{0.97} & \textbf{0.01} & 86.45 & 7.77 & 24.76 & \textbf{78.10} & 45.52 & \textbf{80.31} & 87.97 & 7.00 & \textbf{4.33} & 10.00 & 6.00 & 6.83 \\ 
    Reflextion & 1.37 & 0.22 & 94.71 & 8.19 & 26.40 & 76.73 & 45.73 & \underline{80.28} & \underline{89.96} & 10.00 & 7.00 & 9.00 & \textbf{2.00} & 7.00 \\ 
    MAC & 3.55 & 3.73 & 97.68 & 9.61 & \textbf{31.46} & 75.47 & 42.11 & 79.98 & 88.38 & 11.00 & 7.67 & 11.00 & 7.00 & 9.17 \\ 
    MAD & 1.37 & 0.16 & 91.77 & 7.81 & \underline{26.42} & 76.26 & 46.27 & 79.05 & \textbf{90.14} & 9.00 & 7.00 & 7.00 & 6.00 & 7.25 \\ 
    \hdashline[0.5pt/1pt]
    RAG ($M$=8) & 3.95 & 0.08 & 84.92 & \textbf{5.99} & 20.80 & 76.94 & 56.00 & 79.91 & 89.09 & 5.00 & 5.33 & \textbf{1.00} & 7.00 & 4.58 \\ 
    RAG ($M$=4) & 2.81 & 0.07 & 83.67 & 6.10 & 21.02 & 76.77 & 53.60 & 79.99 & 89.68 & 4.00 & 6.33 & 4.00 & \underline{3.00} & \underline{4.33} \\ 
    RAG ($M$=1) & 2.53 & \underline{0.06} & 85.36 & 6.56 & 22.68 & 77.00 & 50.43 & 79.79 & 89.55 & 6.00 & \underline{4.67} & 6.00 & 5.50 & 5.54 \\ 
    RAG + Extr. ($M$=4) & 3.33 & 0.09 & 83.60 & \underline{6.05} & 21.06 & 76.70 & \textbf{54.66} & 79.73 & 89.30 & 3.00 & 6.67 & \underline{2.00} & 8.50 & 5.04 \\ 
    RAG + Extr. ($M$=1) & 3.18 & 0.09 & \underline{82.42} & 6.62 & 22.57 & 76.77 & 52.23 & 79.83 & 89.38 & \underline{2.00} & 6.67 & 5.00 & 6.00 & 4.92 \\ 
    RAG + Abst. & 3.97 & 0.22 & \textbf{81.96} & 6.60 & 22.91 & 76.86 & \underline{54.44} & 79.36 & 89.42 & \textbf{1.00} & 5.33 & 3.00 & 7.50 & \textbf{4.21} \\ 
    \hline
    \multicolumn{15}{c}{DeepSeek-R1} \\ 
    \hline
    Direct & \textbf{0.55} & \textbf{0.01} & 68.78 & \textbf{3.07} & 22.94 & 76.68 & 50.27 & 80.68 & 91.7 & 7.00 & 4.67 & 7.00 & 6.50 & 6.29 \\ 
    \hdashline[0.5pt/1pt]
    RAG ($M$=8) & 2.31 & 0.03 & \textbf{65.31} & 3.94 & \underline{23.30} & \underline{77.21} & \underline{53.87} & \textbf{82.47} & 92.66 & \textbf{1.00} & \underline{3.00} & \underline{2.00} & \textbf{2.00} & \textbf{2.00} \\ 
    RAG ($M$=4) & 1.62 & 0.03 & 66.76 & 3.78 & \textbf{23.37} & 76.95 & 53.02 & \underline{82.00} & 92.45 & 5.00 & \textbf{2.67} & 4.00 & 4.00 & 3.92 \\ 
    RAG ($M$=1) & \underline{1.23} & 0.04 & 66.42 & \underline{3.73} & 22.97 & \textbf{77.37} & 51.82 & 81.54 & \underline{92.89} & 3.00 & \underline{3.00} & 6.00 & 3.50 & 3.88 \\ 
    RAG + Extr. ($M$=4) & 2.00 & 0.03 & 66.45 & 4.04 & 23.28 & 76.94 & 53.69 & \underline{82.00} & 92.66 & 4.00 & 4.33 & 3.00 & \underline{2.50} & 3.46 \\ 
    RAG + Extr. ($M$=1) & 1.25 & 0.03 & \underline{66.19} & 3.76 & 23.23 & 76.94 & 51.95 & 81.66 & \textbf{93.02} & \underline{2.00} & 3.67 & 5.00 & \underline{2.50} & \underline{3.29} \\ 
    RAG + Abst. & 2.04 & \underline{0.02} & 67.57 & 4.96 & 23.16 & 76.63 & \textbf{54.28} & 80.5 & 92.6 & 6.00 & 6.33 & \textbf{1.00} & 6.00 & 4.83 \\ 
    \bottomrule
    \end{tabular}}
    \vspace{-15pt}
    \label{table:main}
\end{table*}

A summary of the proposed evaluation metrics is presented in \tabref{table:metric}. 
Further details regarding the metrics are provided in \appref{appendix:metrics} and the prompts are showed in \appref{appendix:prompt_evaluation}.
While the application of LLM-as-a-Judge has gained recognition in various related studies~\cite{tang2024itinera,singh2024personal,jiang2024towards}, we also conduct human evaluation on a subset of data instances to validate the proficiency of LLM-based assessments, as elaborated in \appref{appendix:human}.

==> sections/benchmark_old_2.tex <==
\section{TravelPlanRAG}

\begin{figure*}[ht]
\centering
\includegraphics[width=\textwidth]{figs/main.png}
\vspace{-18pt}
\caption{Dataset construction pipeline.}
\vspace{-15pt}
\label{figure:main}
\end{figure*}

In this section, we first formalize our travel planning problem in \secref{section:problem}.
Then we introduce our benchmark including data construction \secref{section:data} and method evaluation \secref{section:evaluation}.

\subsection{Background}
\label{section:problem}

% To validate the spatiotemporal planning capabilities of LLM agents, we simplify the travel planning problem into the generation of a single-city, multi-day travel plan consisting of attraction POIs.
% Also, we adopt the sole-planning mode~\cite{xie2024travelplanner} free from tool calls, thereby exclusively assessing the planning skills of the agents.
We delineate some critical definitions below:

\noindent\textbf{Query}.
A travel query $q$ is articulated by the tourist user in natural language, which comprises significant elements such as city name, travel duration, and personalized travel constraints.

\noindent\textbf{Point-of-Interest (POI)}.
A Point-of-Interest (POI) $p=(p_n, p_s, p_t, p_d)$ refers to a specific real-time location that holds significance or interest for travelers, wherein the attributes include the POI name $p_n$, spatial details $p_s$ (\eg address, geocoordinates), temporal references $p_t$ (\eg shopping hours, recommended visit time, expected visit duration), and POI's semantic description $p_d$.
The candidate POIs dependent on the query $q$ are defined as $P^q=\{p^q_i\}_{i=1}^{|P^q|}$.

\noindent\textbf{Online Trajectory}.
An online trajectory is extracted from the retrieved travel-related Web document, which is denoted as $t=(p_{n,1}, p_{n,2},...,p_{n,|t|})$ with only POI names.
And we define the trajectories relevant to the query $q$ as $T^q=\{t^q_i\}_{i=1}^{|T^q|}$.

\begin{prob}
\textbf{Travel Planning}. 
Given a user query $q$, query-dependent POI candidates $P^q=\{p^q_i\}_{i=1}^{|P^q|}$, and query-relevant online trajectories $T^q=\{t^q_i\}_{i=1}^{|T^q|}$, 
the travel plan $s=[(p^q_{n,1},t_{s,1},t_{e,1}),...,(p^q_{n,|s|},t_{s,|s|},t_{e,|s|})]$ is derived by LLM agents via $s=A(q,P^q,T^q)$, where $t_s,t_e$ respectively denote the scheduled start and end time of the POI visit.
\end{prob}

\subsection{Dataset Construction Pipeline}
\label{section:data}

As illustrated in \figref{figure:main}, the construction pipeline of our dataset consists of the following steps:
(1) query generation; (2) POI collection; (3) trajectory collection; culminating in a (4) quality control procedure, which are detailed below.

\noindent\textbf{Query Generation.} 
While the TravelPlanner series~\cite{xie2024travelplanner} has advanced the accessibility of travel query data, its reliance on highly complex user queries diverges from real-world scenarios where travelers often initiate their planning with concise, under-specified demands. 
For instance, users frequently express needs through brief inputs like \textit{3 days in Beijing with a relaxed schedule} in search engines, expecting systems to infer and fulfill implicit requirements.
To bridge this gap between idealized planning tasks and practical applications, our benchmark prioritizes short, realistic queries which mirror common user behavior, while enabling precise alignment with Web trajectories retrievable via search engines that facilitate our retrieval-augmented planning task.

Specifically, we first sample the latest user queries from the data sessions in Baidu search engine\footnote{\url{https://www.baidu.com}}, one of China’s largest search engines.
Taking these queries as seeds, we engage the LLM to generate a comprehensive query dataset.

To demonstrate the diversity of our queries, we begin with several fundamental elements, including the city name, travel duration, and personal constraints reflecting user preferences. 
Our query framework adopts a multidimensional classification system to ensure comprehensive coverage of various planning scenarios.
In particular, queries are primarily categorized into generic and personal types based on the presence of personalized constraints. 
Personal queries are further classified by constraint types encompassing seasonal preferences, holiday-specific requirements, POI category restrictions, traveler demographics, and trip compactness parameters.
Besides, the travel duration the query instances into short-term, medium-term, and long-term intervals.
The details of query data are presented in \appref{appendix:query}
This orthogonal combinations of constraint dimensions and temporal scales can systematically test LLM agent’s capabilities in handling different user focuses and planning horizons. 

\noindent\textbf{POI Collection.}
To gather attraction POI candidates and associated attribute information for each query, we resort to LLMs augmented by search engines.
Specifically, we exploit the query rewriting strategy~\cite{ma2023query}, leveraging the LLM to reformulate original queries into POI-level sub-queries tailored for attraction recommendations.
The Baidu search engine is utilized to retrieve pertinent documents for each sub-query.
The documents generally contain a lot of irrelevant snippets, thereby we apply the LLM to extract the POI information within each document.
To obviate noisy and hallucinated POIs, we subsequently adopt Baidu Map platform\footnote{\url{https://lbsyun.baidu.com/}} to standardize these POIs into unified names, alongside enhancing them with complete spatial information such as address and geocoordinates. 

Furthermore, spatiotemporal-aware travel planning necessitates fine-grained temporal information and contextual semantics. 
Thus, for each query-POI pair (\eg \textit{Plan a spring trip in Beijing. - the Great Wall}), we craft real-time inquiries (\eg \textit{What's the recommended travel time period of the Great Wall in spring?}) to search related documents about this POI.
Then the retrieval-augmented LLM is harnessed to summarize the nuanced temporal and semantic insights for spatiotemporal planning, which include shopping hours, recommended visit time, expected visit duration, and semantic POI description.

\noindent\textbf{Trajectory Collection.}
Similarly, to collect the online knowledge, we first retrieve up-to-date documents about real-life travel experiences relevant to the given query.
To address user privacy concerns, full documents are not disclosed in our dataset. 
Instead, we implement a LLM-based desensitization process through exactly distilling the tourist trajectories from the original lengthy documents.
To ensure faithfulness, we also instruct the LLM to abstain from answering if the document is not enclosed with any plausible trajectory-level information.
To emulate the retrieval noise commonly found in real-world scenarios, we retain the disturbances present in these trajectories.
Anyway, as introduced in the quality control stage below, we also prepare a denoised version of trajectory data for further in-depth analysis.

\noindent\textbf{Quality Control.}
To ensure the quality of the generated dataset, we apply both LLM and human evaluators to perform a review of all \textit{query-POI-trajectory} data instances and eliminate the semantic noise in POIs and trajectories.
Instances without sufficient trajectory references are discarded.
This procedure guarantees the feasibility of our retrieval-augmented spatiotemporal travel planning task.

To conclude, our dataset consists of 2,348 travel queries including 115 generic queries and 2,233 personal queries. 
This dataset is associated with 85,575 attraction POIs (averaging 36.45 POIs per request) derived from 5,018 unique attractions, and 18,784 retrieved trajectories (averaging 8 trajectories per request). 
Throughout the data construction process, we utilized GPT-4o~\cite{hurst2024gpt}, and the prompts employed are presented in \appref{appendix:prompt_data_generation}.

\subsection{Evaluation}
\label{section:evaluation}

Beyond merely measuring the compliance with hard constraints in travel plans, we shed light on the nuanced aspects of generated plans, particularly concerning spatiotemporal rationality and the semantic prominence of POIs. 
In contrast to TripCraft~\cite{chaudhuri2025tripcraft}, we conceptualize spatiotemporal travel planning as a multi-objective optimization problem, without unique optimal solutions, limiting the reliability of annotating golden plans.
Following existing works~\cite{tang2024itinera,chen2024travelagent}, our evaluation framework integrates rule-based metrics alongside LLM-as-a-Judge methodologies, emphasizing five critical evaluation dimensions: commonsense, spatial, temporal, POI semantic and query relevance. 
This approach effectively circumvents costly annotations and mitigates potential evaluation biases, with metric descriptions provided below.

\noindent\textbf{Commonsense.}
Commonsense metrics measure whether the generated plan adhere to basic plan validity, including:
\textit{(1) Failure Rate (FR)}: the percentage of legitimate POIs without hallucination;
\textit{(2)Repetition Rate (RR)}: the frequency of POI repetition in the plan.

\noindent\textbf{Spatial.}
The spatial metric evaluates the route efficiency of the plan.
Specifically, we use \textit{Distance Margin Ratio (DMR)} to quantify the distance gap from the optimal route calculated via the Traveling Salesman Problem (TSP) solver\footnote{\url{https://github.com/fillipe-gsm/python-tsp}}.

\noindent\textbf{Temporal.}
Temporal metrics aim to assess the rationality of the scheduled tourist periods of POIs, which embrace 
\textit{(1) Start Time Rationality (STR)}: whether the arranged arrival time for POI visit is appropriate;
\textit{(2) Duration Underflow Ratio (DUR)}: the extent to which the planned schedule meets expectations;
\textit{(3) Time Buffer Ratio (TBR)}: the proportion of buffer time available throughout the plan which indicates the degree of tourist comfort.

\noindent\textbf{POI Semantic.}
The semantic metric examines how popular and distinctive the selected POIs are.
In particular, we design a \textit{POI Popularity (PP)} metric measuring the recall rate within the retrieved attraction leaderboard.

\noindent\textbf{Query Relevance.}
The relevance metrics focus on whether the user requirements specified in the queries are fulfilled, which can be divided into two aspects:
\textit{(1) POI Relevance (PR)}: the alignment between planned POIs and the user query;
\textit{(2) Time Schedule Relevance (TSR)}: the pertinence of the arranged POI visit period and personalized needs.

\begin{table*}[ht]
    \centering
    \vspace{-10pt}
    \caption{Main results (\%) of different methods on our dataset. $M$ denotes the number of online trajectories we use for RAG. $R_S$, $R_T$, $R_P$, $R_R$ and $R_C$ respectively denotes the performance rank of methods from spatial, temporal, POI semantic and query relevance dimensions, and a comprehensive view averaging all aspects.}
    \vspace{-8pt}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l|cc|ccccccc|cccc|c}
    \toprule
    \textbf{Method} & \textbf{FR$\downarrow$} & \textbf{RR$\downarrow$} & \textbf{DMR$\downarrow$} & \textbf{DUR$\downarrow$} & \textbf{TBR$\uparrow$} & \textbf{STR$\uparrow$} & \textbf{PP$\uparrow$} & \textbf{PR$\uparrow$} & \textbf{TSR$\uparrow$} & $R_S\downarrow$ & $R_T\downarrow$ & $R_P\downarrow$ & $R_R\downarrow$ & $R_C\downarrow$ \\ 
    \hline
    \multicolumn{15}{c}{GPT-4o} \\ 
    \hline
    Direct & \textbf{0.32} & \textbf{0.00} & 67.92 & 3.03 & 22.01 & 77.22 & 50.82 & 80.51 & \underline{92.52} & 6.00 & 7.67 & 7.00 & \textbf{3.00} & 5.92 \\ 
    CoT & \underline{0.39} & \underline{0.01} & 69.4 & 2.78 & 22.13 & 76.96 & 50.09 & 79.92 & 91.99 & 8.00 & 8.00 & 10.00 & 6.50 & 8.12 \\ 
    Reflextion & 0.67 & 0.34 & 73.35 & 3.84 & 21.46 & 77.3 & 50.52 & 80.34 & \textbf{92.71} & 10.00 & 8.67 & 8.00 & \underline{3.50} & 7.54 \\ 
    MAC & 1.40 & 0.72 & 66.11 & 3.67 & \textbf{24.07} & 75.41 & 46.38 & \textbf{81.76} & 89.04 & 3.00 & 7.00 & 11.00 & 6.00 & 6.75 \\ 
    MAD & 0.68 & 0.07 & 74.95 & 3.68 & 20.67 & 77.14 & 50.52 & 79.53 & 92.4 & 11.00 & 9.67 & 8.00 & 6.50 & 8.79 \\ 
    \hdashline[0.5pt/1pt]
    RAG ($M$=8) & 2.05 & \underline{0.01} & 68.37 & 2.57 & \underline{23.82} & 77.19 & \underline{58.00} & \underline{80.55} & 91.58 & 7.00 & 4.67 & \underline{2.00} & 5.00 & 4.67 \\ 
    RAG ($M$=4) & 2.08 & 0.02 & 67.75 & 2.55 & 23.71 & 77.35 & 56.11 & 80.53 & 91.67 & 5.00 & 3.67 & 4.00 & 4.50 & \underline{4.29} \\ 
    RAG ($M$=1) & 2.43 & 0.04 & \underline{66.05} & 2.47 & 22.59 & 77.44 & 53.38 & 80.1 & 91.5 & \underline{2.00} & 4.00 & 6.00 & 8.50 & 5.12 \\ 
    RAG + Extr. ($M$=4) & 1.91 & 0.02 & 66.99 & \textbf{2.41} & 23.5 & \textbf{77.87} & 56.82 & 80.31 & 91.69 & 4.00 & \textbf{2.00} & 3.00 & 6.00 & \textbf{3.75} \\ 
    RAG + Extr. ($M$=1) & 2.72 & 0.06 & \textbf{65.76} & \underline{2.42} & 22.95 & \underline{77.79} & 53.85 & 80.39 & 91.64 & \textbf{1.00} & \underline{3.00} & 5.00 & 6.00 & \textbf{3.75} \\ 
    RAG + Abst. & 3.20 & 0.02 & 69.49 & 2.64 & 22.23 & 76.66 & \textbf{59.15} & 79.36 & 90.67 & 9.00 & 7.67 & \textbf{1.00} & 10.50 & 7.04 \\ 
    \hline
    \multicolumn{15}{c}{Qwen2.5-72B-Instruct} \\ 
    \hline
    Direct & \textbf{0.38} & \textbf{0.03} & 71.67 & 6.49 & 24.82 & 78.33 & 48.53 & 79.68 & 92.86 & 8.00 & \underline{5.00} & 8.00 & 9.00 & 7.50 \\ 
    CoT & \underline{0.42} & \underline{0.04} & 70.51 & 6.64 & 24.66 & 78.77 & 47.09 & 80.12 & 93.16 & 7.00 & 5.33 & 10.00 & 8.00 & 7.58 \\ 
    Reflextion & 2.39 & 1.62 & 85.38 & 8.08 & 25.37 & 77.54 & 49.15 & 79.65 & 92.14 & 10.00 & 7.67 & 7.00 & 10.00 & 8.67 \\ 
    MAC & 1.10 & 2.21 & 70.08 & \textbf{5.74} & 23.65 & 76.48 & 43.3 & \underline{81.28} & 90.00 & 6.00 & 7.33 & 11.00 & 6.50 & 7.71 \\ 
    MAD & 3.30 & 1.49 & 87.47 & 9.46 & \textbf{26.53} & 77.75 & 47.49 & 80.23 & 91.21 & 11.00 & 7.00 & 9.00 & 9.00 & 9.00 \\ 
    \hdashline[0.5pt/1pt]
    RAG ($M$=8) & 3.41 & 0.11 & 69.39 & \underline{6.35} & 23.48 & 78.4 & \underline{55.15} & \textbf{81.67} & 93.29 & 5.00 & 6.00 & \underline{2.00} & \underline{3.00} & 4.00 \\ 
    RAG ($M$=4) & 3.15 & 0.11 & 68.77 & 6.54 & 24.06 & \textbf{79.08} & 53.62 & 81.26 & \textbf{93.86} & 3.00 & \underline{5.00} & 4.00 & \textbf{2.00} & \textbf{3.50} \\ 
    RAG ($M$=1) & 2.58 & 0.09 & \textbf{68.07} & 6.89 & 25.27 & 78.48 & 51.62 & 81.07 & 93.4 & \textbf{1.00} & 5.33 & 6.00 & 4.50 & 4.21 \\ 
    RAG + Extr. ($M$=4) & 3.46 & 0.16 & 69.03 & 6.49 & 24.33 & \underline{79.03} & 54.79 & 81.21 & \underline{93.81} & 4.00 & \textbf{4.33} & 3.00 & \underline{3.00} & \underline{3.58} \\ 
    RAG + Extr. ($M$=1) & 3.16 & 0.20 & \underline{68.29} & 6.73 & \underline{25.59} & 78.33 & 52.36 & 80.92 & 93.42 & \underline{2.00} & \underline{5.00} & 5.00 & 4.50 & 4.12 \\ 
    RAG + Abst. & 3.78 & 0.17 & 72.4 & 7.32 & 25.11 & 78.04 & \textbf{56.14} & 80.5 & 93.29 & 9.00 & 7.33 & \textbf{1.00} & 6.00 & 5.83 \\
    \hline
    \multicolumn{15}{c}{LLaMA3.3-70B-Instruct} \\ 
    \hline
    Direct & \textbf{0.67} & \textbf{0.01} & 90.55 & 7.41 & 24.14 & \underline{77.07} & 46.27 & 79.75 & 89.32 & 8.00 & \underline{4.67} & 7.00 & 7.50 & 6.79 \\ 
    CoT & \underline{0.97} & \textbf{0.01} & 86.45 & 7.77 & 24.76 & \textbf{78.10} & 45.52 & \textbf{80.31} & 87.97 & 7.00 & \textbf{4.33} & 10.00 & 6.00 & 6.83 \\ 
    Reflextion & 1.37 & 0.22 & 94.71 & 8.19 & 26.40 & 76.73 & 45.73 & \underline{80.28} & \underline{89.96} & 10.00 & 7.00 & 9.00 & \textbf{2.00} & 7.00 \\ 
    MAC & 3.55 & 3.73 & 97.68 & 9.61 & \textbf{31.46} & 75.47 & 42.11 & 79.98 & 88.38 & 11.00 & 7.67 & 11.00 & 7.00 & 9.17 \\ 
    MAD & 1.37 & 0.16 & 91.77 & 7.81 & \underline{26.42} & 76.26 & 46.27 & 79.05 & \textbf{90.14} & 9.00 & 7.00 & 7.00 & 6.00 & 7.25 \\ 
    \hdashline[0.5pt/1pt]
    RAG ($M$=8) & 3.95 & 0.08 & 84.92 & \textbf{5.99} & 20.80 & 76.94 & 56.00 & 79.91 & 89.09 & 5.00 & 5.33 & \textbf{1.00} & 7.00 & 4.58 \\ 
    RAG ($M$=4) & 2.81 & 0.07 & 83.67 & 6.10 & 21.02 & 76.77 & 53.60 & 79.99 & 89.68 & 4.00 & 6.33 & 4.00 & \underline{3.00} & \underline{4.33} \\ 
    RAG ($M$=1) & 2.53 & \underline{0.06} & 85.36 & 6.56 & 22.68 & 77.00 & 50.43 & 79.79 & 89.55 & 6.00 & \underline{4.67} & 6.00 & 5.50 & 5.54 \\ 
    RAG + Extr. ($M$=4) & 3.33 & 0.09 & 83.60 & \underline{6.05} & 21.06 & 76.70 & \textbf{54.66} & 79.73 & 89.30 & 3.00 & 6.67 & \underline{2.00} & 8.50 & 5.04 \\ 
    RAG + Extr. ($M$=1) & 3.18 & 0.09 & \underline{82.42} & 6.62 & 22.57 & 76.77 & 52.23 & 79.83 & 89.38 & \underline{2.00} & 6.67 & 5.00 & 6.00 & 4.92 \\ 
    RAG + Abst. & 3.97 & 0.22 & \textbf{81.96} & 6.60 & 22.91 & 76.86 & \underline{54.44} & 79.36 & 89.42 & \textbf{1.00} & 5.33 & 3.00 & 7.50 & \textbf{4.21} \\ 
    \hline
    \multicolumn{15}{c}{DeepSeek-R1} \\ 
    \hline
    Direct & \textbf{0.55} & \textbf{0.01} & 68.78 & \textbf{3.07} & 22.94 & 76.68 & 50.27 & 80.68 & 91.7 & 7.00 & 4.67 & 7.00 & 6.50 & 6.29 \\ 
    \hdashline[0.5pt/1pt]
    RAG ($M$=8) & 2.31 & 0.03 & \textbf{65.31} & 3.94 & \underline{23.30} & \underline{77.21} & \underline{53.87} & \textbf{82.47} & 92.66 & \textbf{1.00} & \underline{3.00} & \underline{2.00} & \textbf{2.00} & \textbf{2.00} \\ 
    RAG ($M$=4) & 1.62 & 0.03 & 66.76 & 3.78 & \textbf{23.37} & 76.95 & 53.02 & \underline{82.00} & 92.45 & 5.00 & \textbf{2.67} & 4.00 & 4.00 & 3.92 \\ 
    RAG ($M$=1) & \underline{1.23} & 0.04 & 66.42 & \underline{3.73} & 22.97 & \textbf{77.37} & 51.82 & 81.54 & \underline{92.89} & 3.00 & \underline{3.00} & 6.00 & 3.50 & 3.88 \\ 
    RAG + Extr. ($M$=4) & 2.00 & 0.03 & 66.45 & 4.04 & 23.28 & 76.94 & 53.69 & \underline{82.00} & 92.66 & 4.00 & 4.33 & 3.00 & \underline{2.50} & 3.46 \\ 
    RAG + Extr. ($M$=1) & 1.25 & 0.03 & \underline{66.19} & 3.76 & 23.23 & 76.94 & 51.95 & 81.66 & \textbf{93.02} & \underline{2.00} & 3.67 & 5.00 & \underline{2.50} & \underline{3.29} \\ 
    RAG + Abst. & 2.04 & \underline{0.02} & 67.57 & 4.96 & 23.16 & 76.63 & \textbf{54.28} & 80.5 & 92.6 & 6.00 & 6.33 & \textbf{1.00} & 6.00 & 4.83 \\ 
    \bottomrule
    \end{tabular}}
    \vspace{-15pt}
    \label{table:main}
\end{table*}

Further details regarding the metrics are provided in \appref{appendix:metrics} and the prompts for evaluation are showed in \appref{appendix:prompt_evaluation}.
% While the application of LLM-as-a-Judge has gained recognition in various related studies~\cite{tang2024itinera,singh2024personal,jiang2024towards}, we also conduct human evaluation on a subset of data instances to validate the proficiency of LLM-based assessments, as elaborated in \appref{appendix:human}.

==> sections/experiment_old_1.tex <==
\section{Experiment}

\subsection{Baselines}

\noindent\textbf{Planning Strategies.}
We evaluate various planning strategies as follows:
\textsl{(1) Planning from scratch}: 
Besides direct prompting, we test advanced planning strategies including Chain-of-Thoughts (CoT)~\cite{wei2022chain} and Reflextion~\cite{shinn2023reflexion}, to probe the capability of LLM agents.
Inspired by related multi-agent planning methods, we implement Multi-Agent Collaboration (MAC) which applies divide-and-conquer solution~\cite{zhang2025planning}, and Multi-Agent Debate (MAD) that launches a discussion session for plan refinement~\cite{ni2024planning}.
\textsl{(2) Retrieval-augmented planning}:
To explore the potential of plan improvements by incorporating itinerary-level knowledge on the Web, we assess the LLM agents equipped with the RAG approach. 
We additionally consider two simple prompt-based post-retrieval techniques: \textit{extractive and adstractive compression}~\cite{xu2024recomp}, which are expected to further purify the retrieved content for possible enhancements.
The implementation of baselines and other evaluation details are presented in \appref{appendix:setup}.
For DeepSeek-R1, we only rely on its reasoning ability without applying complex planning strategies.

\noindent\textbf{Base Models.}
We conduct our experiments on various LLMs including a proprietary foundation model: GPT-4o~\cite{hurst2024gpt}, two open-source foundation models: Qwen2.5-72B-Instruct~\cite{yang2024qwen2}, LLaMA3.3-70B-Instruct~\cite{llama}, and an open-source reasoning-optimized model: DeepSeek-R1~\cite{guo2025deepseek}.

\subsection{Main Results}
\label{section:main}

In this section, we discuss the performances of different models and strategies on our TravelPlanRAG benchmark as illustrated in \tabref{table:main}.
We summarize our observations as follows:

\noindent\textbf{Advanced LLM agents struggle with spatiotemporal-aware travel planning.}
Across the results of three foundation models, cutting-edge strategies (\ie CoT, Reflextion and multi-agent techniques) all underperform compared to direct prompting as evidenced by the holistic ranking $R_C$. 
This reveals that complex task decomposition or answer reflection can instead lead to error accumulation and a degeneration of spatiotemporal perception, highlighting the inherent challenges in fine-grained travel planning.

\noindent\textbf{Online knowledge holds great potential to foster LLM-based travel planning.}
According to the multifaceted metric $R_C$ applied to various base models, retrieval-augmented planning methodologies generally demonstrate a significant advantage over LLM agent planning from scratch, underscoring the value of integrating external knowledge for effective travel planning.
The performance gain primarily derives from enhancements in spatial and POI semantic dimensions, while there is a slight decline in some models regarding the temporal aspect (concerning LLaMA3.3) and relevance (in relation to LLaMA and GPT-4o). 
This can be attributed to the agents’ limited capacity to comprehend confusing web content.

\noindent\textbf{Sophisticated strategies negatively affect agents' commmonsense awareness.}
While the overall impact is not severe, we observe a notable increase in inaccessible or repetitive POIs within both advanced LLM planning strategies and RAG-based strategies. 
This trend indicates the risks associated with violating commonsense constraints when employing intricate methodologies, wherein LLMs are perplexed by long-context and complicated inputs.

\noindent\textbf{Reasoning-optimized LLMs fail to stay ahead as expected in travel planning.}
Despite the rapid rise of reasoning-enhanced models such as Deepsek-R1, which we anticipated would significantly outperform earlier foundational models (e.g., GPT, Qwen, and LLaMA series)~\cite{valmeekam2024llms}, it yields unsatisfactory outcomes in our spatiotemporal travel planning task, particularly lagging in the temporal dimension.

\noindent\textbf{Retrieval-augmented planning methods lack stability.}
It is noteworthy that richer external knowledge and elegant post-retrieval processing methods do not guarantee superiority, showcasing inconsistent effectiveness across various base models. 
We defer an in-depth analysis to \secref{section:rag}.

\noindent\textbf{Performances of distinct evaluation dimensions are inconsistent.}
There is no single solution that consistently ranks high across all evaluation dimensions. 
Trade-offs between different metrics are commonly observed in most cases. 
% We analyze the relationships among various assessment dimensions in \secref{section:metric_relation} for further discussion.

\begin{table*}[h!]
    \centering
    % \vspace{-10pt}
    \caption{Comparison between EvoRAG and baseline methods on our dataset implemented by Qwen2.5-72B-Instruct. 
    % $M$ denotes the number of external itineraries we use for RAG. $R_S$, $R_T$, $R_P$, $R_R$ and $R_C$ respectively denotes the performance rank of methods from 4 dimensions: spatial, temporal, POI semantic and query relevance, and a comprehensive view averaging the former four aspects.
    }
    \vspace{-8pt}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l|cc|ccccccc|cccc|c}
    \toprule
    \textbf{Method} & \textbf{FR$\downarrow$} & \textbf{RR$\downarrow$} & \textbf{DMR$\downarrow$} & \textbf{DUR$\downarrow$} & \textbf{TBR$\uparrow$} & \textbf{STR$\uparrow$} & \textbf{PP$\uparrow$} & \textbf{PR$\uparrow$} & \textbf{TSR$\uparrow$} & $R_S\downarrow$ & $R_T\downarrow$ & $R_P\downarrow$ & $R_R\downarrow$ & $R_C\downarrow$ \\ 
    \hline
    Direct & \textbf{0.38} & \textbf{0.03} & 71.67 & 6.49 & 24.82 & 78.33 & 48.53 & 79.68 & 92.86 & 9.00 & 5.67 & 9.00 & 9.50 & 8.29 \\
    CoT & 0.42 & \underline{0.04} & 70.51 & 6.64 & 24.66 & 78.77 & 47.09 & 80.12 & 93.16 & 8.00 & 6.33 & 11.00 & 8.50 & 8.46 \\
    Reflextion & 2.39 & 1.62 & 85.38 & 8.08 & 25.37 & 77.54 & 49.15 & 79.65 & 92.14 & 11.00 & 8.67 & 8.00 & 11.00 & 9.67 \\
    MAC & 1.10 & 2.21 & 70.08 & \textbf{5.74} & 23.65 & 76.48 & 43.3 & 81.28 & 90.00 & 7.00 & 8.00 & 12.00 & 7.50 & 8.62 \\
    MAD & 3.30 & 1.49 & 87.47 & 9.46 & \underline{26.53} & 77.75 & 47.49 & 80.23 & 91.21 & 12.00 & 8.00 & 10.00 & 10.00 & 10.00 \\
    \hdashline[0.5pt/1pt]
    RAG (M=8) & 3.41 & 0.11 & 69.39 & \underline{6.35} & 23.48 & 78.40 & 55.15 & \underline{81.67} & 93.29 & 6.00 & 6.67 & 3.00 & \underline{3.50} & 4.79 \\
    RAG (M=4) & 3.15 & 0.11 & 68.77 & 6.54 & 24.06 & \underline{79.08} & 53.62 & 81.26 & \textbf{93.86} & 4.00 & 5.67 & 5.00 & \textbf{2.50} & \underline{4.29} \\
    RAG (M=1) & 2.58 & 0.09 & \underline{68.07} & 6.89 & 25.27 & 78.48 & 51.62 & 81.07 & 93.40 & \underline{2.00} & 6.33 & 7.00 & 5.00 & 5.08 \\
    RAG + Extr. (M=4) & 3.46 & 0.16 & 69.03 & 6.49 & 24.33 & 79.03 & 54.79 & 81.21 & \underline{93.81} & 5.00 & \underline{5.00} & 4.00 & \underline{3.50} & 4.38 \\
    RAG + Extr. (M=1) & 3.16 & 0.20 & 68.29 & 6.73 & 25.59 & 78.33 & 52.36 & 80.92 & 93.42 & 3.00 & 6.00 & 6.00 & 5.00 & 5.00 \\
    RAG + Abst. & 3.78 & 0.17 & 72.40 & 7.32 & 25.11 & 78.04 & \underline{56.14} & 80.50 & 93.29 & 10.00 & 8.33 & \underline{2.00} & 6.50 & 6.71 \\
    EvoRAG & \underline{0.40} & 0.06 & \textbf{44.45} & 6.54 & \textbf{28.22} & \textbf{81.63} & \textbf{58.05} & \textbf{85.82} & 92.19 & \textbf{1.00} & \textbf{2.33} & \textbf{1.00} & 5.00 & \textbf{2.33} \\
    \bottomrule
    \end{tabular}}
    \vspace{-15pt}
    \label{table:method}
\end{table*}

\subsection{Query Analysis}

In this section, we investigate the results derived from our sub-dataset across various request categories, as illustrated in \figref{figure:radar_gpt}, \figref{figure:radar_qwen}, \figref{figure:radar_llama}, and \figref{figure:radar_deepseek}. 
The analysis reveals that retrieval-augmented strategies significantly outperform ground-up methods, such as direct prompting, across most evaluation metrics. 
This observation aligns with the findings from our full-scale experiments detailed in \secref{section:main}.

\subsection{RAG Analysis}
\label{section:rag}

% \subsubsection{RAG Necessity Analysis}

% \subsubsection{Robustness Analysis}

In this section, we take Qwen2.5-72B-Instruct as an example and investigate the sensitivity of retrieval-augmented planning strategies in relation to the volume and quality of retrieval data, as illustrated in \tabref{table:rag}.
Our observations indicate that performance peaks when $M$ equals 6 or 7. 
Retaining few number of itineraries (i.e., $M<6$) results in a significant decline in performance. 
This underscores the notion that travel planning lacks unique solutions and emphasizes the necessity for diverse plans.
Conversely, utilizing all retrieved results (i.e., $M=8$) presents challenges in assimilating diverse solutions and filtering out low-quality references, despite their relevance to user requests.

Considering the noisy POI data in online itineraries, we evaluate two scenarios: noisy and clean, with the latter benefiting from our denoising operation in \secref{section:data}. 
The overall trend reveals that purifying external knowledge enhances retrieval-augmented planning, improving both commonsense awareness (\ie failure rate) and nuanced spatiotemporal planning, particularly for methods utilizing post-retrieval techniques.

% \subsubsection{RAG utilization Analysis}

% \subsection{Metric Analysis}
% \label{section:metric_relation}


==> sections/introduction_old_1.tex <==
\section{Introduction}

Emerging studies have explored the potential of Large Language Models (LLMs) to serve as travel agents capable of interpreting natural language inquiries and delivering comprehensive travel plans through thoughtful reasoning and planning~\cite{wong2023autonomous}.
Travel planning benchmarks such as TravelPlanner~\cite{xie2024travelplanner}, have gained recognition for assessing LLMs’ capabilities in complex and realistic planning.
Building on these benchmarks, subsequent studies have enhanced LLM-based travel agents~\cite{zhang2025planning,hao2024large,yuan2024evoagent}, even achieving an unprecedented $100$\% success rate in TravelPlanner~\cite{lee2025evolving}. 
Despite the fruitful progress made so far, two critical gaps persist in current travel planning benchmarks, as illustrated in \figref{figure:motivation} and detailed below.

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figs/motivation.png}
\caption{Illustrations of two research gaps.}
\label{figure:motivation}
\end{figure}

\textit{(1) Lack of a reliable spatiotemporal evaluation framework.} 
Current assessments of benchmarks are limited to basic commonsense constraints (\eg complete information, unrepeated POIs), specifically, they are primarily concerned with whether the agents can provide a plan without evident structure and  commonsense failures~\cite{xie2024travelplanner}. 
However, a practical travel plan in real-world applications must extend beyond these elementary factors, integrating deeper consideration such as spatiotemporal coherence of itineraries and the semantic quality of POIs~\cite{tang2024itinera,chen2024travelagent}. 
This raises the question: \textit{Are advanced LLM-based agents capable of travel planning with sufficient spatiotemporal awareness}. 
Initial efforts by ITINERA~\cite{tang2024itinera}, TravelAgent~\cite{chen2024travelagent} and TripCraft~\cite{chaudhuri2025tripcraft} have begun to address this evaluation, yet a thorough and reliable framework for spatiotemporal and semantic validation remain under-explored, which this paper aims to investigate.

\textit{(2) Underutilization of online knowledge for travel planning.}
Existing benchmarks mainly focus on crafting travel plans by LLMs from scratch by selecting and organizing POIs from pre-existing candidates~\cite{xie2024travelplanner}. 
Nevertheless, LLMs have been criticized to suffer from hallucinations~\cite{huang2025survey}, outdated knowledge~\cite{gao2023retrieval}, and deficient spatiotemporal reasoning abilities~\cite{manvi2024geollm,li2024reframing,chu2024timebench}, hindering their capacity to generate desirable plans.
In fact, numerous online travel itineraries are readily available on the Web, reflecting latest real-life experience within spatiotemporal contexts, which could significantly forward travel planning. 
However, risks associated with online information, such as verbose narratives, conflicting solutions, and nonsensical itineraries, can complicate this process.
Thus, we pose a question: \textit{Can LLM agents benefit from itineraries on the Web in spatiotemporal travel planning?} We propose employing Retrieval-Augmented Generation (RAG) techniques to explore this further.

We introduce \textbf{TravelPlanRAG}, a travel planning benchmark which features a new real-world dataset comprising online itineraries from Web, and a rigorous evaluation framework for assessing spatiotemporal efficacy. 
Our data contains 2,348 travel instances (115 generic requests + 2,233 constraint-driven personal requests) across 30 destinations in Chinese mainland, which also cover 85,575 geotagged POIs (5,018 distinct attractions) with density of 36.45 POIs/request, and 18,784 retrieved online itineraries averaging 8 references/request.
For fine-grained assessments, we design a multi-dimension evaluation system spanning 5 perspectives: \textit{commonsense, spatial, temporal, POI semantic and query relevance}, which integrates rule-based metrics and LLM-as-a-Judge~\cite{zheng2023judging}, free from manual annotations. 

\TODO{Experiments}

\TODO{Method}

\TODO{Contribution}










==> sections/introduction_old_2.tex <==
\section{Introduction}

Emerging studies have explored the potential of Large Language Models (LLMs) to serve as travel agents capable of interpreting natural language inquiries and delivering comprehensive travel plans through thoughtful reasoning and planning~\cite{wong2023autonomous}.
However, existing benchmarks such as TravelPlanner~\cite{xie2024travelplanner} primarily focus on whether the provided plans satisfy basic commonsense requirements (\eg complete information, truly existent POIs), 
neglecting nuanced rationality (\eg spatiotemporal coherence, POI semantic quality).
This oversight limits their practical applicability in real-world scenarios.

In this paper, we delve into \textit{spatiotemporal travel planning}, to investigate LLM agents' capabilities of spatiotemporal perception and planning.
Despite their promise, LLMs encounter challenges such as hallucinations~\cite{huang2025survey}, outdated knowledge~\cite{gao2023retrieval}, and deficient spatiotemporal reasoning abilities~\cite{manvi2024geollm,li2024reframing,chu2024timebench}.
These issues hinder the effectiveness of LLMs in independently crafting elaborate travel plans from scratch. 
We refer to this approach as \textit{ground-up spatiotemporal travel planning}.
Intriguingly, numerous travel itineraries are readily accessible on the Web, reflecting latest real-life experience within spatiotemporal contexts, which hold substantial potential for fine-grained travel planning. 
However, risks associated with online information, such as verbose narratives, conflicting solutions, and nonsensical itineraries, can complicate this endeavor.
Thus, we raise a question: \textit{Can LLM agents benefit from online itineraries in spatiotemporal travel planning?} 
To explore this, we propose employing Retrieval-Augmented Generation (RAG) techniques, and propose the paradigm \textit{retrieval-augmented spatiotemporal travel planning}. 
A comparison of different planning paradigms is illustrated in  \figref{figure:motivation}.

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figs/motivation.png}
\vspace{-20pt}
\caption{Illustrations of different paradigms.}
\vspace{-23pt}
\label{figure:motivation}
\end{figure}

To advance the investigation above, we introduce \textit{TravelPlanRAG}, a travel planning benchmark which features a new real-world dataset allowing for retrieval-augmented spatiotemporal travel planning.
In contrast to datasets available in previous works, relying on Retrieval-Augmented LLMs (RALLMs), TravelPlanRAG incorporates rich spatiotemporal information into POI contexts, and integrates plentiful online knowledge from the Web via Baidu Search\footnote{\url{https://www.baidu.com}}, one of China’s largest search engines.
Generally, our data contains 2,348 travel instances (115 generic requests + 2,233 constraint-driven personal requests) across 30 destinations in Chinese mainland, covering 85,575 geotagged POIs (5,018 distinct attractions) with density of 36.45 POIs/request, and 18,784 retrieved online itineraries averaging 8 references/request.
In addition, for spatiotemporal assessments, we establish a comprehensive evaluation system spanning 5 perspectives: commonsense, spatial, temporal, POI semantic and query relevance, which integrates rule-based metrics and LLM-as-a-Judge~\cite{zheng2023judging}, free from manual annotations. 

We evaluate various planning strategies across two spatiotemporal planning paradigms and four cutting-edge LLMs. 
The results expose notable limitations in advanced ground-up LLM planning methods, while presenting promising prospects for the utilization of online knowledge despite limited performance stability.
Furthermore, our RAG analysis uncovers concerns about the robustness of retrieval-augmented planning approaches.

To address the challenges of retrieval-augmented travel planning, we propose \textit{EvoTravel}, a LLM-based evolutionary optimization framework designed to effectively blend the advantages of diverse retrieved knowledge with the agents’ internal knowledge, while alleviating the impact of insufficient information. 
Our experiments demonstrate the superiority of this methodology.

Our main contributions are three-fold:
(1) To the best of our knowledge, we propose \textit{TravelPlanRAG}, the first travel planning benchmark tailored for retrieval-augmented travel planning with spatiotemporal awareness. 
This benchmark includes a dataset characterized by diverse request data, copious itinerary-level knowledge and rich POI corpus with spatiotemporal contexts, and a comprehensive automated evaluation system.
(2) We conduct extensive experiments on various planning strategies and advanced LLMs, revealing the opportunities and challenges of retrieval-augmented travel planning.
(3) We introduce \textit{EvoTravel}, a new method that unleash the power of retrieval-augmented LLM agents for spatiotemporal travel planning.











==> sections/introduction_old_3.tex <==
\section{Introduction}

Emerging studies have explored the potential of Large Language Models (LLMs) to serve as travel agents capable of interpreting natural language inquiries, and autonomously generating travel plans that comprise daily tourist activities detailed with various Points of Interest (POIs)~\cite{wong2023autonomous}.
% Theses agents interpret natural language inquiries, adaptively consult external travel-related knowledge and then deliver optimized plans through thoughtful reasoning and planning.
Despite their promise, existing works~\cite{xie2024travelplanner,singh2024personal,hao2024large} focus primarily on whether the generated plans meet basic commonsense requirements (\eg complete information, actual POIs), while overlooking the nuanced spatiotemporal rationality that is critical for practicality. 
Key aspects include (1) spatiotemporal coherence (\eg optimizing the transit efficiency and time buffers between POIs), (2) POI appealingness (\ie ensuring recommended landmarks reflect local cultural characteristics and popularity), and (3) real-time demands (\ie time-evolving POI information, such as seasonal closures and altered opening hours).
These oversights may result in flawed plans characterized by inefficient routes, exhausting journeys, unappealing POIs, or limited adaptability. Therefore, this study investigates the capabilities of LLM agents in travel planning while emphasizing spatiotemporal awareness.

\begin{figure}[ht]
\centering
\includegraphics[width=\linewidth]{figs/motivation.pdf}
\vspace{-24pt}
\caption{TP-RAG distinguishes itself from existing works by: (1) real-time spatiotemporal contextualization and (2) trajectory knowledge utilization.}
\vspace{-18pt}
\label{figure:motivation}
\end{figure}

Contemporary research primarily focuses on benchmarking the abilities of LLM agents in travel planning~\cite{xie2024travelplanner,singh2024personal} or exploring sophisticated strategies to enhance planning effectiveness~\cite{tang2024itinera,xie2024human}.
However, these studies rely exclusively the candidate POIs, and agents’ internal reasoning capabilities to construct travel plans from scratch.
This ground-up approach faces inherent limitations stemming from insufficient spatiotemporal reasoning~\cite{manvi2024geollm,li2024reframing,chu2024timebench} and the generation of hallucinated or outdated content~\cite{huang2025survey,gao2023retrieval}, which restrict the spatiotemporal coherence of the produced travel plans.
Intriguingly, beyond the point-level knowledge concerning POIs, the Web contains a wealth of up-to-date travel documents that encode spatiotemporally contextualized insights into real-life tourist trajectories, representing the line-level knowledge.
The advancements in Retrieval-augmented Generation (RAG) approaches~\cite{fan2024survey} enable LLM agents to integrate these online trajectories for potential spatiotemporal improvements.

In this paper, we introduce a new travel planning benchmark, \textit{TP-RAG}, to investigate whether LLM agents can effectively leverage the online knowledge at the trajectory level to produce coherent spatiotemporally travel plans.
Our benchmark features a dataset grounded in real-world data sources, constituted of 2,348 travel queries, 85,575 geotagged POIs and 18,784 online trajectory references.
It is designed to develop and evaluate LLM agents in generating coherent spatiotemporal travel plans tailored for the queries, utilizing relevant POIs and trajectories.
Unlike prior datasets, our dataset incorporates real-time spatiotemporal contexts into POI information, enabling time-adaptive and spatiotemporal-aware planning.
In addition, the inclusion of tourist trajectories encourages retrieval-augmented LLM agents to employ the vast repository of online knowledge for plan enhancements.
The comparison between \textit{TP-RAG} and existing works is illustrated in \figref{figure:motivation}.

Based on our benchmark, we evaluate various LLM-based travel planning methods.
The experimental results reveal notable limitations of advanced LLM agents which are constrained by internal knowledge, while also highlighting promising prospects for the utilization of online knowledge.
Our in-depth analysis further uncovers concerns regarding the universality and robustness of Web-augmented travel planning approaches.
To address these challenges, we propose \textit{EvoRAG}, a LLM-based evolutionary framework that iteratively optimizes the travel plans through population-based selection, crossover and mutation of retrieved online knowledge.
It effectively blends the advantages of diverse retrieved knowledge and the agents’ intrinsic planning capacity, while alleviating the impact of insufficient information, the superiority of which is demonstrated by our experiments.

Our main contributions are three-fold:
(1) We propose \textit{TP-RAG}, the first travel planning benchmark for retrieval-augmented and spatiotemporal-aware travel planning, characterized by diverse query data, a rich POI corpus with spatiotemporal contexts, and extensive trajectory knowledge.
(2) We introduce \textit{EvoRAG}, a new method that further promotes retrieval-augmented LLM agents for spatiotemporal travel planning.
(3) We conduct extensive experiments on various travel planning methods in various evaluation dimensions, showcasing both the opportunities and challenges of incorporating trajectory-level knowledge and manifesting the preeminence of our method.











==> sections/method_old_1.tex <==
\section{EvoRAG}

To address the aforementioned issues, we advance the capabilities of retrieval-augmented travel agents through a LLM-based evolutionary algorithm.
Refer \appref{appendix:method} for the detailed algorithm workflow.
Following existing works~\cite{yuan2024evoagent,lee2025evolving}, we propose \textit{EvoRAG}, which emphasizes three key improvements:
First, for population initialization, we generate $|T|$ initial solutions individually from all trajectories and include an additional solution derived solely from direct prompting. 
This attains an ensemble of retrieval-augmented and ground-up planning aimed at optimized efficacy.
Second, after solution evaluation, we employ LLMs to assess their strengths and weaknesses based on evaluation feedback, guiding deliberate reflection on the plan population from distinct perspectives.
Third, based on evaluation, we retain the best $\alpha$ proportion of parent solutions solely for mutation, 
meanwhile selecting dissimilar parents to perform crossover and mutation, until we obtain $(|T|+1)$ solutions. 
This strategy ensures a balance between effectiveness and diversity, consolidating varied retrieved knowledge while minimizing noise interference.
The prompts used are shown in \appref{appendix:prompt_method}.

\begin{figure}[ht]
    \centering
    \vspace{-10pt}
    \includegraphics[width=0.7\linewidth]{figs/method.pdf}
    \vspace{-8pt}
    \caption{Comparison of EvoRAG and baselines.}
    \vspace{-10pt}
    \label{figure:method}
\end{figure}

Taking the Qwen model as an example, \textit{EvoRAG} generally surpasses both ground-up and retrieval-augmented planning methods across almost all dimensions (except for query relevance $R_R$), as illustrated in \figref{figure:method}.
\textit{EvoRAG} also achieves notable reductions in commonsense failures, with 0.4\% POI failure rate (FR) and 0.06\% POI repetition rate (RR), which are comparable to the \textit{Direct} baseline.
The complete experimental results are provided in \appref{appendix:method}.
This further underscores the proficiency of integrating trajectory-level knowledge with LLM-based optimization, paving the way for future advancements in LLM-driven travel agents.




==> sections/preliminary.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth]{figs/main.png}
\caption{Dataset construction pipeline.}
\label{figure:main}
\end{figure*}

\section{Preliminary}

In this section, we present a formal introduction to our proposed travel planning problem. 
In contrast to prior works such as TravelPlanner~\cite{xie2024travelplanner}, our focus is directed towards validating the spatiotemporal planning capabilities of LLM agents. 
To this end, we simplify the travel planning problem into the generation of a single-city, multi-day travel itinerary, which comprises a selection of attraction POIs.
Furthermore, we adopt a sole-planning mode that obviates the need for tool calls, thereby exclusively assessing the planning skills of the agents~\cite{xie2024travelplanner}.
We frame the travel planning problem as a multi-objective optimization task, as delineated below:

\begin{prob}
\textbf{Travel Planning}. 
Given a travel request $r$ articulated in natural language along with pre-determined POI candidates $\mathcal{P}=\{p_i\}_{i=1}^{N}$, the LLM agent $\mathcal{L}$ selects a subset of POIs and organizes them into a plan $I=[(p_1,t_1),(p_2,t_2),...,(p_M,t_M)]$ via $I\sim\mathcal{L}(r,\mathcal{P})$, where $t$ denotes the visiting period planned in the itinerary. The generated plan $I$ is expected to align with the request $r$ while maximizing spatiotemporal coherence and POI semantic quality.
\end{prob}

To further enhance the potential of our approach, we propose the concept of \textit{\textbf{Retrieval-Augmented Travel Planning}}, depicted as $I\sim\mathcal{L}(r,\mathcal{P}, \mathcal{K})$.
This allows for the incorporation of online knowledge $\mathcal{K}=\{k_i\}_{i=1}^{M},\ k_i=[p_1,p_2,...,p_{|k_i|}]$ as auxiliary resources, thereby enriching the planning process with current and relevant information from the Web.

==> sections/related_work_old_1.tex <==
\section{Related Work}

\subsection{LLM Agent for Travel Planning}

A pivotal contribution to language-driven automated travel planning is TravelPlanner~\cite{xie2024travelplanner}, which benchmarks language agents on long-horizon and multi-constraint travel planning tasks, revealing the limitations faced by LLMs in addressing these complex scenarios.
Subsequent studies have sought to enhance planning efficacy through advanced LLM strategies, such as multi-agent collaboration techniques~\cite{xie2024human,zhang2025planning}, external solvers~\cite{de2024trip,ju2024globe,hao2024large}, and LLM-as-an-optimizer techniques~\cite{yanglarge,yuan2024evoagent}, which can achieve an impressive 100\% success rate through evolutionary optimization methods~\cite{lee2025evolving}.
Some other works set out to establish LLM-based travel planning systems for real-world applications~\cite{tang2024itinera,chen2024travelagent}.

\subsection{Benchmarks of LLM-based Travel Planning}

Recent advancements in LLM-based travel planning have led to the emergence of several benchmark studies, notably inspired by TravelPlanner~\cite{xie2024travelplanner}. 
These benchmarks target specific scenarios, demonstrating the evolving capabilities of LLM agents.
For instance, TravelPlanner+~\cite{singh2024personal} explores LLM agents' abilities in personalized travel planning 
by integrating individual user profiles.
Ask-before-Plan~\cite{zhang2024ask} examines how LLM agents manage ambiguous instructions through proactive user interaction.
Moreover, several studies benchmark neural-symbolic travel planning frameworks that combine LLMs with external solvers, such as PDDL and SMT solvers~\cite{hao2024large,de2024trip,shao2024chinatravel}. 
However, existing benchmarks frequently overlook spatiotemporal rationality, hampering practical applications.
The recent work TripCraft~\cite{chaudhuri2025tripcraft} enriches travel planning with real-world details (\eg transport schedule, travel events) and applies spatiotemporal evaluation. 
Nevertheless, TripCraft does not adequately address nuanced spatiotemporal characteristics at the POI level, and its reliance on subjective human annotations results in biased and unreliable evaluation outcomes. 
This gap highlights the necessity for further study into spatiotemporal travel planning.

% \subsection{Evaluation of LLM-based Travel Planning}

% The assessment of LLMs in travel planning primarily revolves around their ability to produce coherent plans devoid of structural and commonsense failures, as evaluated by rule-based metrics~\cite{xie2024travelplanner}.
% Beyond basic pass rate assessments, various studies have employed LLM-as-a-Judge methodologies and human evaluations to gauge the quality and personalization of generated plans~\cite{singh2024personal,tang2024itinera,chen2024travelagent}.
% However, critical dimensions of rationality, such as spatiotemporal coherence and POI semantic quality, remain inadequately addressed.
% For instance, while ITINERA~\cite{tang2024itinera} emphasizes spatial coherence and POI quality, it overlooks temporal validity. 
% Additionally, TravelAgent~\cite{chen2024travelagent} and fNarritiveGuide~\cite{ding2025narrative} rely on coarse-grained scoring via LLMs or humans, which is inherently subjective and potentially unreliable in quantifying nuanced spatiotemporal attributes.
% TripCraft~\cite{chaudhuri2025tripcraft} neglects semantic quality (\eg POI popularity) but gives a spatiotemporal evaluation protocol by annotating golden itineraries and exploit statistical models to measure the spatiotemporal deviations from the ground-truth distributions.
% Nevertheless, travel planning lacks unique optimal solutions, making manual annotations potentially biased and narrow.
% Also, the assumptions in parametric models may not reflect real-world patterns and heavy human efforts hinder adaptive and portable evaluation.

\subsection{Travel-Domain Retrieval-Augmented Generation}

The emergence of Retrieval-Augmented Generation (RAG) has marked a significant advancement in LLM capabilities, facilitating the integration of external knowledge to enhance generative quality~\cite{fan2024survey}. 
Within the travel domain, preliminary developments have been observed, particularly in travel-related question-answering~\cite{song2024travelrag,yu2025spatial} and POI recommendation~\cite{qi2024rag} tasks. 
Nonetheless, the potential application of RAG to augment travel planning with external itinerary-level knowledge remains largely unexplored.

==> sections/related_work_old_2.tex <==
\section{Related Work}

\subsection{Benchmarks of LLM-based Travel Planning}

To assess the capabilities of LLM agents in complex and realistic planning tasks, recent benchmarks have proliferated in travel planning, which stands out as a significant domain.
For example, TravelPlanner~\cite{xie2024travelplanner} establishes foundational investigation for long-horizon travel planning under multi-constraint scenarios, exposing inherent limitations in LLM agents. 
Subsequent extensions like TravelPlanner+~\cite{singh2024personal} incorporate user profiling for personalized tourist plan generation, while Ask-before-Plan~\cite{zhang2024ask} evaluates proactive clarification-seeking behaviors in ambiguous travel query resolution before planning. 
TripCraft~\cite{chaudhuri2025tripcraft} further advances practical applicability by integrating real-world characteristics including transit schedules and tourist events. 
Beyond relying solely on LLMs, another line of benchmarks examine the hybrid approaches  which leverage LLMs for natural language interpretation paired with symbolic solvers to ensure solution validity through formal verification~\cite{hao2024large,de2024trip,shao2024chinatravel}. 
Despite progress, these benchmarks fail to incorporate sufficient fine-grained spatiotemporal contexts into planning, and are constrained by agents' internal knowledge and reasoning process, which hinder the real-world deployment.
Our benchmark addresses these issues by contextualizing real-time spatiotemporal POI details and applying trajectory-level online knowledge to augment practical spatiotemporal-aware travel planning.

\subsection{LLM Agent for Travel Planning}

Travel planning remains an intricate problem entailing intent comprehension, information seeking, long-horizon planning, and personalized customization.
To automate this task, contemporary research on LLM travel agents bifurcates into two paradigms: native and hybrid. 
Native approaches aim to enhance LLM agents' intrinsic planning capacities.
Some works employ multi-agent collaboration to achieve enhanced travel itinerary design through sophisticated coordination mechanisms, where distinct sub-agents specialize in decomposing complex problem and resolving separate sub tasks~\cite{xie2024human,zhang2025planning}.
Other works harness LLM-based optimization techniques to iteratively refine the quality of travel schedules~\cite{yuan2024evoagent,lee2025evolving}.
Contrastingly, hybrid approaches compensate for LLM agents' limitations through integration of computational planning modules.
For instance, ITINERA~\cite{tang2024itinera} strengthens spatial coherence via a route optimization module.
TravelAgent~\cite{chen2024travelagent} pioneers a heuristic planning framework mirroring human cognitive processes in tourist scheduling. 
TTG~\cite{ju2024globe} employs symbolic solvers on task representations translated by fine-tuned LLMs.
To promote the inherent capabilities of travel agents, we propose \textit{EvoRAG} which unifies the rich retrievable knowledge and the internal optimization abilities of LLM agents.

\subsection{Retrieval-Augmented Generation}

Retrieval-Augmented Generation (RAG) systems have emerged as pivotal solutions for enhancing LLMs with external knowledge~\cite{fan2024survey}. 
To evaluate the performances of RAG, recent research efforts have been devoted to building reliable benchmarks, which emphasize two assessment aspects: retrieval efficacy (\eg relevance, utility)~\cite{lyu2025crud,saad2024ares,dai2025seper} and generation quality (\eg accuracy, coherence)~\cite{chen2024benchmarking,qi2024long2rag,tang2024multihop}, where our study focuses on the latter one.
Beyond open-domain scenarios, some studies have demonstrated success in specific domains such as medical, legal and financial fields~\cite{xiong2024benchmarking,pipitone2024legalbench,wang2024omnieval}, 
while travel applications remain nascent, particularly focusing on question-answering (QA)~\cite{song2024travelrag,yu2025spatial} and POI recommendation~\cite{qi2024rag}, restricted in POI-level tasks. 
Besides, comprehensive benchmarks for complex travel planning tasks requiring real-time knowledge integration and multi-objective resolution are underexplored. 
Our work bridges these gaps through trajectory-level retrieval-augmented mechanisms for spatiotemporal travel planning.

